The trace formula and the existence of PEL type Abelian varieties modulo p

We show, using the trace formula, that any Newton stratum of a Shimura variety of PEL-type of types (A) and (C) is non-empty at the primes of good reduction. Furthermore we prove conditionally the non-emptiness for Shimura data associated to odd Spin groups. Our results are conditional on Rapoport-Langlands conjecture and Arthur's conjectures on the discrete spectrum. Both these results have been announced by Arthur and Kisin in significant cases.

==> nonempty_temp.tex <==
%!TEX root = nonempty.tex


NOTE: Deze sectie vervangt de versie van afgl zaterdag. De andere secties heb ik toen al verbeterd. Ik moet dus alleen deze toevoegen.

\bigskip

\section{NEW: Symplectic groups}

Let $G$ be a group of a Shimura datum satisfying the conditions from \S 1, and additionally the following: We have an exact sequence $[G_1 \injects G \surjects \Gm]$, where $G_1$ is an inner form of a symplectic group over a totally real extension $F^+$ of $\Q$. We call the morphism $G \surjects \Gm$ the factor of similitudes. We show that $G$ satisfies Hypothesis~\ref{hypG} under these assumptions completing the proof of the nonemptiness for PEL varieties of type C.

Using results of Arthur we show that Hypothesis~\ref{hypG} is true for $G$. Arthur recently proved his conjecture for the group $G_1^*$. This is sufficient information for us. We write $G^*$ (resp. $G_1^*$) for the quasi-split inner form of $G$ (resp. $G_1$). The dual group $\widehat {G_1^*}$ is a product of $[F^+:\Q]$ copies of the group $\SO_{2g+1}(\C)$, with the absolute Galois group acting by permutation of the factors. We write ${}^LG_1^* := \SO_{2g+1}(\C)^{[F^+:\Q]} \rtimes \cG_\Q$. We recall briefly the result of Arthur for the group $G_1^*$. Let $\pi$ be a discrete automorphic representation of the group $G_1^*$. Arthur associates to $\pi$ a parameter $\psi \colon \cL_{\Q} \times \SU_2(\R) \to {}^{L} G_1^*$, where $\cL_\Q$ is the conjectural\footnote{We refer to \cite[\S 1.3]{arthurbook} for the explanation how these statement can be made independent of conjectures (at the cost of some technical burden). Roughly, one replaces the parameters $\psi$ with essentially self-dual cuspidal automorphic representations of $\Gl_N$.} global Langlands group of $\Q$. These $L$-parameters $\psi$ are determined (up to conjugation) by the set of its local components $\psi_v \colon \cL_{\Q_v} \times \SU_2(\R) \to {}^{L} G_1$, where $v$ ranges over a (any) set of places \emph{with finite complement}, where $\cL_{\Q_v}$ is the local Langlands group. Using endoscopy Arthur parametrizes the elements of the packet $\Pi(\psi)$. Write, if $v$ is a $\Q$-place, $\cG_{\Q_v}$ for the absolute Galois group of $\Q_v$. For each place $v$ define $\widehat \cS_{\psi, v} := \Hom(\textup{Cent}_{\widehat G}(\psi) / \textup{Cent}_{\widehat G}(\psi)^\circ Z(\widehat G)^{\cG_{\Q_v}}, \C^\times)$. For each element of the packet $\pi_v \in \Pi(\psi_v)$, there is a character $\langle \cdot, \pi_v \rangle \in \widehat \cS_{\phi, v}$. In the tempered case, the characters in $\widehat \cS_{\psi}$ parametrize the elements of the local packets $\Pi(\psi_v)$. The global packet $\Pi(\psi)$ is the set of restricted tensor products $\pi = \bigotimes_v^\prime \pi_v$ such that
\begin{itemize}
\item $\pi_v \in \Pi(\psi_v)$;
\item The representation $\pi_v$ is unramified for nearly all $v$. 
\end{itemize}
Arthur defines the subset $\Pi(\psi)(\eps_{\psi}) \subset \Pi(\psi)$ consisting of those $\pi$ such that additionally:
\begin{itemize}
\item The product $\prod_v \langle \cdot, \pi_v \rangle$ is equal to a certain~\cite[p.~47]{arthurbook} explicit character $\eps_{\psi}$ depending only on the parameter $\psi$. 
\end{itemize}
Then he proves that $\Pi(\psi)(\eps_{\psi})$ is precisely the set of $\pi \in \Pi(\psi)$ occurring in the discrete spectrum of $G_1$. Arthur also computes the multiplicities (they turn out to be 1), but we will not need that fact.

\begin{theorem}[Conditional]\label{hyptruegsp}
Hypothesis~\ref{hypG} is true for the group $G$.
\end{theorem}
\begin{remark}
The theorem depends on the results in the book of Arthur. In turn those results depend on the stabilization of the twisted trace formula for $\Gl_n$. Therefore the theorem is conditional on this stabilization as well. 
\end{remark}
\begin{proof}[Proof of Theorem~\ref{hyptruegsp}.]
Let $(\Pi, \Pi_0)$ be a couple of cuspidal automorphic representations of the group $G$, satisfying the conditions of Hypothesis~\ref{hypG}. By assumption, the representation $\Pi_v$ is a twist of $\Pi_{0, v}$ at the places $v \in \Sigma := \{x_1, \ldots, x_r, p_1, p_2\}$. We must show that $\Pi_p$ is an unramified twist of $\Pi_{0, p}$. To simplify notations, we assume in the rest of the proof $\Pi_v \cong \Pi_{0, v}$. Furthermore, we only have to prove a property of automorphic representations of the quasi-split inner forms of $(G_1, G)$. Thus, to simplify notations, we can assume that $G_1$ and $G$ are already quasi-split. 

By Proposition~\ref{st:extension} there exist cuspidal automorphic representations\footnote{The cuspidal automorphic $G_1(\A)$-subrepresentations $\pi$ of $\Pi$ are by no means unique or canonical; in fact in most of the cases we expect there to be an infinite number of discrete automorphic $\pi \subset \Pi$. See the remark below Proposition TO DO. } $\pi, \pi_0$ of $G_1$ contained in $\Pi, \Pi_0$. Let $\psi$ and $\psi_0$ be the Arthur parameters for $\pi$ and $\pi_0$. The representations $\pi, \pi_0$ are automorphic, and thus unramified outside a finite set of places\footnote{Note that the set of ramification of $\pi, \pi_0$ may be larger than the set of ramification of $\Pi, \Pi_0$}. %: Let $y$ be a place where $\Pi_y$ is unramified, so that it has an $K_y$-invariant vector with $K_y$ hyperspecial in $G(\Q_y)$. Put $K_{1, y} := K_1 \cap G_1(\Q_y)$. The restriction of $\Pi_y$ to $G_1(\Q_y)$ is a direct sum of finitely many irreducible representations $\pi_i$. Assume $0 \neq v \in \pi_i$ is $K_{1, y}$ spherical vector. The representations $\pi_i$ are spherical for groups of the form $g_i G_1(\Z_y) g_i^{-1}$, with $g_i \in G(\Q_y)$. }
We know that $\Pi$ and $\Pi_0$ are isomorphic outside a finite set, and furthermore, a local unramified representation of $G(\Q_v)$ (for some $v$) contains exactly one unramified representation of $G_1(\Q_v)$. Hence $\pi$ and $\pi_0$ are representations in the cuspidal spectrum which are isomorphic outside a finite set of places. Consequently $\pi$ and $\pi_0$ have the same Arthur parameter: $\psi \colon \cL_\Q \times \SU_2(\R) \to {}^L G_1$. We have $\pi_p, \pi_{0, p} \in \Pi(\psi_p)$. We look at the auxiliary place $p_1$. By assumption, the representation $\Pi_{0, p_1}$ is (a finite twist of) the Steinberg representation of $G(\Q_{p_1})$. By Lemma~\ref{surprise}.(\textit{i}) the restriction of $\Pi_{0, p_1}$ to $G_1(\Q_{p_1})$ is \emph{irreducible} and isomorphic to (a twist of) the Steinberg representation. Thus $\pi_{0, p_1}$ is a twist of the Steinberg representation. Therefore $\psi_{p_1}$ is tempered, and the restriction of the parameter $\psi$ to the $\SU_2(\R)$-factor is trivial [TO DO]. The second $\SU_2(\R)$-factor of the local parameter 
$$
\psi_p \colon \underset {\cL_{\Q_p}}{\underbrace{\cW_{\qp} \times \SU_2(\R)}} \times \SU_2(\R) \to {}^L G_1,
$$
is therefore trivial as well. Thus we have the more fine information that $\pi_p, \pi_{0, p}$ lie in the same Langlands packet. The representation $\pi_{0, p}$ is a subrepresentation of $\Pi_{0, p} = \Ind_{P(\qp)}^{G(\qp)}(\St_{M(\qp)}(\chi))$ for some standard parabolic subgroup $P$ of $G_{\qp}$.

We have the following lemma:

\begin{lemma}\label{surprise}
Let $M \subset G_{\qp}$ be a standard Levi-subgroup. Let $M_1 \subset M$ be the kernel of the morphism of similitudes. Let $\St_{M(\qp)}(\chi)$ be an unramified unitary twist of the Steinberg representation of $M(\qp)$.
\begin{itemize}
\item[(\textit{i})] 
The restriction of the representation $\St_{M(\qp)}$ to $M_1$ is irreducible. 
\item[(\textit{ii})] The restriction of the induced representation $\Ind_{P(\qp)}^{G(\qp)}(\St_{M(\qp)})$ to $G_1(\qp)$ is irreducible and isomorphic to $\Ind_{P_1(\qp)}^{G_1(\qp)}(\St_{M_1(\qp)}(\chi'))$, where $\chi'$ is the restriction of $\chi$ to $M_1(\qp)$. 
\end{itemize}
\end{lemma}

(The lemma is proved at the end of this section.)
\smallskip

Consequently $\pi_{0, p}$ is an induction of the form $\Ind_{P_1(\qp)}^{G_1(\qp)}(\St_{M_1(\qp)})$. The Steinberg representation $\St_{M_1(\qp)}$ is the unique representation in its packet, and the parabolic induction of a tempered packet is again a packet. Since $\pi_p$ lies in the same packet as $\pi_{0, p}$, and this packet is a singleton, we get $\pi_p \cong \pi_{0, p}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{surprise} (i).]
In this proof we identify groups with their sets of $\qp$-rational points (we write $G, M, P, \ldots$, where we should have written $G(\qp), M(\qp), \ldots$). Let $B$ be the standard Borel subgroup of $M$, and write $B_1 := B \cap M_1$. We show that $M/B \isomto M_1/B_1$. We have the sequence $S_1 := [B_1 \injects B \surjects \qpm]$ mapping into the sequence $S_2 := [M_1 \injects M \rightarrow \qpm]$. Let us check that $B \rightarrow \qpm$ is surjective\footnote{The map $M \rightarrow \qpm$ is surjective as well, but we do not need that fact.}: We may decompose $B = TN$, $B_1 = T_1 N$, where $T_1$ the diagonal torus of $M_1$, $T$ the diagonal torus of $M$, and $N$ is the unipotent part (which is the same for $B$ and $B_1$). To check that $B \to \qpm$ is surjective, it suffices to check that $T \surjects \qpm$. To see that $T \surjects \qpm$, it suffices that $H^1(\qp, T_{1,\qp})$ vanishes. The torus $T_1$ is the restriction of scalars of a split torus, thus $H^1(\qp, T_{1,\qp})$ vanishes by Shapiro and Hilbert 90. Thus $B \rightarrow \qpm$ is surjective as claimed. By easy diagram chase we get from the morphism $S_1 \rightarrow S_2$ that $M/B = M_1/B_1$. Thus we have an $M_1$-equivariant isomorphism $C^\infty(M/B) \isomto C^\infty(M_1/B_1)$ between the locally constant complex valued functions on $M/B$ and $M_1/B_1$. This isomorphism induces a bijection from $\St_M$ to $\St_{M_1}$. Consequently, the restriction of $\St_M$ to $M_1$ is irreducible.

Proof of (\textit{ii}). The representation $\pi := \Ind_{M_1(\qp)}^{G_1(\qp)}(\St_{M_1(\qp)}(\chi))$ occurs in $\Pi := \Ind_{M(\qp)}^{G(\qp)}(\St_{M(\qp)}(\chi))$. We know that 
$$
\pi \supset \St_{M_1(\qp)}(\chi) \cong \St_{M(\qp)}(\chi) \subset \Pi
$$ 
\end{proof}
